MatFormer: A Generative Model for Procedural Materials

Procedural material graphs are a compact, parameteric, and resolution-independent representation that are a popular choice for material authoring. However, designing procedural materials requires significant expertise and publicly accessible libraries contain only a few thousand such graphs. We present MatFormer, a generative model that can produce a diverse set of high-quality procedural materials with complex spatial patterns and appearance. While procedural materials can be modeled as directed (operation) graphs, they contain arbitrary numbers of heterogeneous nodes with unstructured, often long-range node connections, and functional constraints on node parameters and connections. MatFormer addresses these challenges with a multi-stage transformer-based model that sequentially generates nodes, node parameters, and edges, while ensuring the semantic validity of the graph. In addition to generation, MatFormer can be used for the auto-completion and exploration of partial material graphs. We qualitatively and quantitatively demonstrate that our method outperforms alternative approaches, in both generated graph and material quality.

==> sections/metadata.tex <==
\title{\name: A Generative Model for Procedural Materials}

\author{Paul Guerrero}
\email{guerrero@adobe.com}
\orcid{0000-0002-7568-2849}

% \affiliation{
%   \institution{Adobe Research}
%   \city{London}
%   \country{UK}
% }

\author{Milo\v{s} Ha\v{s}an}
\email{mihasan@adobe.com}
\orcid{0000-0003-3808-6092}

\affiliation{
  \institution{Adobe Research}
}

\author{Kalyan Sunkavalli}
\email{sunkaval@adobe.com}
\orcid{0000-0002-6030-2348}

\author{Radom\'{i}r M\v{e}ch}
\email{rmech@adobe.com}
\orcid{0000-0002-5558-0327}

% \affiliation{
%   \institution{Adobe Research}
%   \city{San Jose}
%   \country{USA}
% }

\author{Tamy Boubekeur}
\email{boubek@adobe.com}
\orcid{0000-0001-5985-0921}

% \affiliation{
%   \institution{Adobe Research}
%   \city{Paris}
%   \country{France}
% }

\affiliation{
  \institution{Adobe Research}
}

\author{Niloy J. Mitra}
\email{n.mitra@cs.ucl.ac.uk}
\orcid{0000-0002-2597-0914}

\affiliation{
  \institution{Adobe Research}
%   \city{London}
%   \country{UK}
}
\affiliation{
  \institution{University College London}
%   \city{London}
%   \country{UK}
}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Guerrero et al.}


\input{sections/abstract.tex}

%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010382</concept_id>
<concept_desc>Computing methodologies~Image manipulation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010257</concept_id>
<concept_desc>Computing methodologies~Machine learning</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Image manipulation}
\ccsdesc[300]{Computing methodologies~Machine learning}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{node graphs, procedural materials, transformers, generative models}

